Jointly Discovering Visual Objects and Spoken Words from Raw Sensory Input

In this paper, we explore neural network models that learn to associate segments of spoken audio captions with the semantically relevant portions of natural images that they refer to. We demonstrate that these audio-visual associative localizations emerge from network-internal representations learned as a by-product of training to perform an image-audio retrieval task. Our models operate directly on the image pixels and speech waveform, and do not rely on any conventional supervision in the form of labels, segmentations, or alignments between the modalities during training. We perform analysis using the Places 205 and ADE20k datasets demonstrating that our models implicitly learn semantically-coupled object and word detectors.

==> retrieval_table_old.tex <==
\begin{table}[htb]
\setlength\tabcolsep{3pt}
\small
  \caption{Recall scores on the held out set of 1,000 images/captions for the three matchmap similarity functions. We also show results for the baseline models which use automatic speech recognition-derived text captions. \textcolor{red}{TODO: clean up the table here, verify that the text follows the table well}}
  \label{tab:retrieval_algos}
  \centering
  \begin{tabular}{ccccccc}
    \toprule
    \multicolumn{1}{c}{} & \multicolumn{3}{c}{Caption to Image} & \multicolumn{3}{c}{Image to Caption}\\
    Model & R@1 & R@5 & R@10 & R@1 & R@5 & R@10 \\
    \cmidrule(lr){2-4}\cmidrule(lr){5-7}
    Speech SISA & .063 & .191 & .274 & .048 & .166 & .249 \\
    Speech MISA & .079 & .225 & .314 & .057 & .191 & .291 \\
    Speech SIMA & .073 & .213 & .284 & .065 & .168 & .255 \\
    \midrule
    (Pretrained) Speech SISA & .165 & .431 & .559 & .120 & .363 & .506 \\
    (Pretrained) Speech MISA & .200 & .469 & .604 & .127 & .375 & .528 \\
    (Pretrained) Speech SIMA & .147 & .375 & .506 & .139 & .367 & .483 \\
    \midrule
    ASR SISA (Text) & .136 & .365 & .503 & .106 & .309 & .430 \\
    ASR MISA (Text) & .162 & .417 & .547 & .113 & .309 & .447 \\
    ASR SIMA (Text) & .134 & .389 & .513 & .145 & .336 & .459 \\
    \midrule
    (Pretrained) ASR SISA (Text) & .230 & .525 & .665 & .174 & .462 & .611 \\
    (Pretrained) ASR MISA (Text) & .271 & .567 & .701 & .183 & .489 & .622 \\
    (Pretrained) ASR SIMA (Text) & .215 & .518 & .639 & .220 & .494 & .599 \\
    \midrule
    \cite{harwath_nips} (Speech) & .148 & .403 & .548 & .121 & .335 & .463 \\
    \cite{harwath_acl_2017} (Speech) & .161 & .404 & .564 & .130 & .378 &  .542 \\
    \bottomrule
  \end{tabular}
\end{table}
